Recurrence Extraction for Functional Programs through Call-by-Push-Value (Extended Version)

The main way of analyzing the complexity of a program is that of extracting and solving a recurrence that expresses its running time in terms of the size of its input. We develop a method that automatically extracts such recurrences from the syntax of higher-order recursive functional programs. The resulting recurrences, which are programs in a call-by-name language with recursion, explicitly compute the running time in terms of the size of the input. In order to achieve this in a uniform way that covers both call-by-name and call-by-value evaluation strategies, we use Call-by-Push-Value (CBPV) as an intermediate language. Finally, we use domain theory to develop a denotational cost semantics for the resulting recurrences.

==> cbpv-extraction-lists.tex <==
\begin{minipage}{0.45\textwidth}
  \begin{align*}
    \potential{\natt}           &\defeq \natt     \\
    \potential{A_1 \times A_2}  &\defeq \potential{A_1} \times \potential{A_2} \\
    \potential{U\ct{B}}         &\defeq \carrier{\complexity{\ct{B}}} \\
    \potential{\plistv{A}}      &\defeq \plist{\potential{A}}
  \end{align*}
\end{minipage}
\begin{minipage}{0.45\textwidth}
  \begin{align*}
    \complexity{FA}                     
      &\defeq (\cost \times \potential{A}, \mu_A) \\
    \complexity{A \rightarrow \ct{B}}     
      &\defeq (\potential{A} \rightarrow \carrier{\complexity{\ct{B}}}, 
               \alpha_{A \rightarrow \ct{B}}) \\
    \complexity{\ct{B}_1 \with \ct{B}_2}  
      &\defeq (\carrier{\complexity{\ct{B}_1}} \times \carrier{\complexity{\ct{B}_2}}, 
              \alpha_{\ct{B}_1 \with \ct{B}_2}) \\
    \complexity{\plistc{\ct{B}}}
      &\defeq (\cost \times \plist{\carrier{\complexity{\ct{B}}}}, \alpha_{\plistc{\ct{B}}})
  \end{align*}
\end{minipage}

\begin{alignat*}{3}
  c : \cost, x : \cost \times \potential{A}
    &\vdash
      \mu_A(c, x)
        &&\defeq 
          \tuple{c \plusc \pi_1(x)}{ \pi_2(x)} 
      &&: \cost \times \potential{A} \\
  c : \cost, f : \potential{A} \rightarrow \carrier{\complexity{\ct{B}}}
    &\vdash
      \alpha_{A \rightarrow\ct{B}}(c, f)
        &&\defeq
          \lambda a.\ \alpha_{\ct{B}}\left(c, f(a)\right)
      &&: \potential{A} \rightarrow \carrier{\complexity{\ct{B}}} \\
  c : \cost, p : \carrier{\complexity{\ct{B}_1}} \times \carrier{\complexity{\ct{B}_2}}
    &\vdash
      \alpha_{\ct{B}_1 \with \ct{B}_2}(c, p)
        &&\defeq
          \tuple
            {\alpha_{\ct{B}_1}(c, \pi_1(p))}
            {\alpha_{\ct{B}_2}(c, \pi_2(p))}
      &&: \carrier{\complexity{\ct{B}_1}} \times \carrier{\complexity{\ct{B}_2}} \\
  c : \cost, p : \cost \times \plist{\carrier{\complexity{\ct{B}}}}
    &\vdash
      \alpha_{\plistc{\ct{B}}}(c, xs)
        &&\defeq
          \tuple{c \plusc \pi_1(p)}
                {\textsf{map}\left(\lambda x.\ \alpha_{\ct{B}}(c, x), \pi_2(p)\right)}
      &&: \cost \times \plist{\carrier{\complexity{\ct{B}}}}
\end{alignat*}

\textbf{Note}: whenever $\Gamma \vdash E : \complexity{FA}$, we
let $ 
  \begin{cases}
    \Gamma \vdash E_c \defeq \pi_1(E) : \cost \\
    \Gamma \vdash E_p \defeq \pi_2(E) : \potential{A}
  \end{cases}
$

\begin{tabular}{ccc}

  %% VARIABLE RULE
  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \cbpvtv{\Gamma, x : A, \Gamma'}{x}{x}{A}
    \using
      {(\textsf{var})}
  \end{prooftree}
  $

  &

  %% NATURALS
  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \cbpvtv{\Gamma}{\numl{n}}{\num{n}}{\natt}
  \end{prooftree}
  $

  &

  % FIXPOINT RULE
  $
  \begin{prooftree}
      \cbpvtc{\Gamma, x : U\ct{B}}{M}{P}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}{\fix{x}{M}}{\fix{x}{P}}{\ct{B}}
  \end{prooftree}
  $

  \\[3ex]

  %% Introduction for value product types
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V_1}{W_1}{A_1}
        \quad
      \cbpvtv{\Gamma}{V_2}{W_2}{A_2}
    \justifies
      \cbpvtv{\Gamma}{(V_1, V_2)}{\tuple{W_1}{W_2}}{A_1 \times A_2}
  \end{prooftree}
  $

  & 

  \multicolumn{2}{c}{
  %% Elimination for value product types
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{P}{A_1 \times A_2}
        \quad
      \cbpvtc{\Gamma, x_1 : A_1, x_2 : A_2}{N}{Q}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}
             {\splitprod{V}{x_1}{x_2}{N}}
             {Q[\pi_1(P)/x_1, \pi_2(P)/x_2]}{\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% Introduction for free type
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{P}{A}
    \justifies
      \cbpvtc{\Gamma}{\return{V}}{\tuple{\zeroc}{P}}{FA}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  %% Elimination for free type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{Q}{FA}
          \quad
      \cbpvtc{\Gamma, x : A}{N}{R}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}
             {\bind{x}{M}{N}}
             {\costof{Q} +_{\ct{B}} R[\potentialof{Q}/x]}
             {\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% Introduction for function type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma, x : A}{M}{P}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}
             {\lambda x.\ M}
             {\lambda x.\ P}
             {A \rightarrow \ct{B}}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  %% Elimination for function type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{P}{A \rightarrow \ct{B}}
        \quad
      \cbpvtv{\Gamma}{N}{Q}{}
    \justifies
      \cbpvtc{\Gamma}{M\,N}{P\,Q}{\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]
  
  %% Introduction for computation product type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{P}{\ct{B}_1}
        \quad
      \cbpvtc{\Gamma}{N}{Q}{\ct{B}_2}
    \justifies
      \cbpvtc{\Gamma}{\tuple{M}{N}}
                     {\tuple{P}
                            {Q}
                     }
                     {\ct{B}_1 \with \ct{B}_2}
  \end{prooftree}
  $

  &

  %% Introduction for thUnk type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{P}{\ct{B}}
    \justifies
      \cbpvtv{\Gamma}{\thunk{M}}{P}{U\ct{B}}
  \end{prooftree}
  $

  &

  %% Elimination for thUnk type
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{P}{U\ct{B}}
    \justifies
      \cbpvtc{\Gamma}{\force{V}}{P}{\ct{B}}
  \end{prooftree}
  $

  \\[3ex]

  %% Elimination for computation product type
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{P}{\ct{B}_1 \with \ct{B}_2}
    \justifies
      \cbpvtc{\Gamma}{\pi_i(M)}{\pi_i(P)}{\ct{B}_i}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{W}{\natt}
    \quad
      \cbpvtc{\Gamma}{M}{P}{\ct{B}}
    \quad
      \cbpvtc{\Gamma}{N}{Q}{\ct{B}}
    \justifies
      \cbpvtv{\Gamma}{\ifz{V}{M}{N}}
                     {\pif{W}{P}{Q}}
                     {\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]

  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{M}{P}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}{\charge{M}}{\unitc +_{\ct{B}} P}{\ct{B}}
  \end{prooftree}
  $

  &

  %% value nil
  $
  \begin{prooftree}
    \justifies
      \cbpvtv{\Gamma}{\nilv}{\nil}{\plistv{A}}
  \end{prooftree}
  $

  &

  %% computation nil
  $
  \begin{prooftree}
    \justifies
      \cbpvtc{\Gamma}{\nilc}{\tuple{\zeroc}{\nil}}{\plistc{\ct{B}}}
  \end{prooftree}
  $

  \\[3ex]

  %% value cons
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{H}{A}
    \quad
      \cbpvtv{\Gamma}{W}{T}{\plistv{A}}
    \justifies
      \cbpvtv{\Gamma}{\consv{V}{W}}{\cons{H}{T}}{\plistv{A}}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  %% computation cons
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{L}{H}{\ct{B}}
    \quad
      \cbpvtc{\Gamma}{K}{T}{\plistc{\ct{B}}}
    \justifies
      \cbpvtc{\Gamma}{\consc{L}{K}}{\tuple{\pi_1(T)}{\cons{H}{\pi_2(T)}}}{\plistc{\ct{B}}}
  \end{prooftree}
  $
  }

  \\[3ex]

  \multicolumn{3}{c}{
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{M}{\natt}
    \quad
      \cbpvtv{\Gamma}{W}{N}{\natt}
    \quad
      \cbpvtc{\Gamma, z : \natt}{P}{Q}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}{\calc{z}{V \cbpvop W}{P}}
                     {Q[M \pcfop N/z]}
                     {\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]

  \multicolumn{3}{c}{
  $
  \begin{prooftree}
      \cbpvtv{\Gamma}{V}{L}{\plistv{A}}
    \quad
      \cbpvtc{\Gamma}{M}{P}{\ct{B}}
    \quad
      \cbpvtc{\Gamma, x : A, xs : \plistv{A}}{N}{P}{\ct{B}}
    \justifies
      \cbpvtc{\Gamma}{\reclistv{V}{M}{x}{xs}{N}}
                     {\reclist{L}{P}{x}{xs}{Q}}
                     {\ct{B}}
  \end{prooftree}
  $
  }

  \\[3ex]

  \multicolumn{3}{c}{
  $
  \begin{prooftree}
      \cbpvtc{\Gamma}{L}{K}{\plistc{\ct{B}}}
    \quad
      \cbpvtc{\Gamma}{M}{P}{\ct{D}}
    \quad
      \cbpvtc{\Gamma, x : U\ct{B}, xs : U\plistc{\ct{B}}}{N}{Q}{\ct{D}}
    \justifies
      \cbpvtc{\Gamma}{\reclistc{L}{M}{x}{xs}{N}}
                     {\reclist{K}{P}{x}{xs}{Q}}
                     {\ct{D}}
  \end{prooftree}
  $
  }

\end{tabular}


==> codestyle.tex <==
% configurations for the listings package

\lstset
{
	tabsize = 2 ,
	showtabs = false ,
  columns=fullflexible,
%	tab = {|} ,
	mathescape ,
  xleftmargin=.25in,
	language = ,
	morekeywords={rec,let,bind,calc,in,return,thunk,force,ifz,if,then,else,val,charge} ,
	sensitive = false ,
	literate={\\}{{$\lambda$}}1 {<-}{{$\leftarrow$ }}2 ,
}


==> cpbv-bigstep-lists.tex <==
\begin{tabular}{ccc}

  %% LAMBDA TERMINAL
  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \eval{\lambda x.\ M}{\lambda x.\ M}{0}
  \end{prooftree}
  $

  &

  %% RETURNER TERMINAL
  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \eval{\return{V}}{\return{V}}{0}
  \end{prooftree}
  $

  & 

  %% TUPLE TERMINAL
  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \eval{\tuple{M}{N}}{\tuple{M}{N}}{0}
  \end{prooftree}
  $

  \\[3ex]

  %% FORCE THUNK
  $
  \begin{prooftree}
      \eval{M}{T}{m}
    \justifies
      \eval{\force{(\thunk{M})}}{T}{m}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  %% SPLIT POSITIVE PRODUCT
  $
  \begin{prooftree}
      \eval{N[V_1/x_1, V_2/x_2]}{T}{m}
    \justifies
      \eval{\splitprod{(V_1, V_2)}{x_1}{x_2}{N}}{T}{m}
  \end{prooftree}
  $
  }

  \\[3ex]

  $
  \begin{prooftree}
      \phantom{\eval{M}{T}{n}}
    \justifies
      \eval{\nilc}{\nilc}{0}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \phantom{\eval{M}{T}{n}}
    \justifies
      \eval{\consc{H}{T}}{\consc{H}{T}}{0}
  \end{prooftree}
  $

  &

  %% FIXPOINT
  $
  \begin{prooftree}
      \eval{M[\thunk{(\fix{x}{M})}/x]}{T}{n}
    \justifies
      \eval{\fix{x}{M}}{T}{n}
  \end{prooftree}
  $

  
  \\[3ex]


  %% IFZ ZERO
  $
  \begin{prooftree}
      \eval{P}{T}{m}
    \justifies
      \eval{\ifz{\numl{0}}{P}{Q}}{T}{m}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  $
  \begin{prooftree}
      \eval{M}{T}{m}
    \justifies
      \eval{\reclistv{\nilv}{M}{x}{xs}{N}}{T}{m}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% IFZ NONZERO
  $
  \begin{prooftree}
      \eval{Q}{T}{m}
    \justifies
      \eval{\ifz{\numl{n+1}}{P}{Q}}{T}{m}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  $
  \begin{prooftree}
      \eval{N[V/x, L/xs]}{T}{m}
    \justifies
      \eval{\reclistv{\consv{V}{L}}{M}{x}{xs}{N}}{T}{m}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% CALC
  $
  \begin{prooftree}
      \eval{P[\numl{m \cbpvop n}/z]}{T}{m}
    \justifies
      \eval{\calc{z}{\numl{m} \cbpvop \numl{n}}{P}}{T}{m}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  $
  \begin{prooftree}
      \eval{L}{\nilc}{n}
    \quad
      \eval{M}{T}{m}
    \justifies
      \eval{\reclistc{L}{M}{x}{xs}{N}}{T}{n + m}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% CHARGE
  $
  \begin{prooftree}
      \eval{M}{T}{n}
    \justifies
      \eval{\charge{M}}{T}{n+1}
  \end{prooftree}
  $

  &

  \multicolumn{2}{c}{
  $
  \begin{prooftree}
      \eval{L}{\consc{H}{T}}{n}
    \quad
      \eval{N[\thunk{H}/x, \thunk{T}/xs]}{T}{m}
    \justifies
      \eval{\reclistc{L}{M}{x}{xs}{N}}{T}{n + m}
  \end{prooftree}
  $
  }

  \\[3ex]

  $
  \begin{prooftree}
      \eval{M}{\return{V}}{m}
        \qquad
      \eval{N[V/x]}{T}{n}
    \justifies
      \eval{\bind{x}{M}{N}}{T}{m + n}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \eval{P}{\tuple{M_1}{M_2}}{m}
        \qquad
      \eval{M_i}{T}{n}
    \justifies
      \eval{\pi_i(P)}{T}{m + n}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \eval{M}{\lambda x.\ P}{m}
        \qquad
      \eval{P[V/x]}{T}{n}
    \justifies
      \eval{M V}{T}{m + n}
  \end{prooftree}
  $

\end{tabular}


==> macros.tex <==
%% this is to get potential brackets
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother


%% AUTHOR MACROS
% general macros
\newcommand{\defeq}{\stackrel{\mathclap{\mbox{\tiny def}}}{=}}
\newcommand{\defiff}{\ \stackrel{\mathclap{\mbox{\tiny def}}}{\equiv}\ }
\newcommand{\aequiv}{\equiv_\alpha}
\newcommand{\dom}{\mathrm{dom} }
\newcommand{\subst}[2]{{#1}\left[#2\right]}
\newcommand{\pcf}{\textsf{PCF}}
\newcommand{\pcfc}{{\textsf{PCF}c}}
\newcommand{\cbpv}{\textsf{CBPV}}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\prog}[1]{\texttt{#1}}

% PCF (source) macros
\newcommand{\pif}[3]{\textsf{if } #1 \textsf{ then } #2 \textsf{ else } #3}
\WithSuffix\newcommand\pif*[3]{%
  \begin{aligned}[t]
  &\textsf{if}\ #1\ \textsf{then}\ #2 \\
  &\textsf{else}\ #3
  \end{aligned}
}
\newcommand{\natt}{\textsf{nat}}
\newcommand{\num}[1]{\underline{#1}}
\newcommand{\fix}[2]{\textsf{fix}\ #1.\ #2}
\newcommand{\fixn}[3]{\textsf{fix}_{#2}\ #1.\ #3}
\newcommand{\rec}[3]{\textsf{rec}\,#1(#2) = #3}
\newcommand{\tuple}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\pcfop}{\mathbin{\textbf{op}}}
\newcommand{\plist}[1]{\left[#1\right]}
\newcommand{\plistv}[1]{\left[#1\right]^{+}}
\newcommand{\plistc}[1]{\left[#1\right]^{-}}
\newcommand{\hd}[1]{\textsf{hd}\left(#1\right)}
\newcommand{\tl}[1]{\textsf{tl}\left(#1\right)}
\newcommand{\nil}{[]}
\newcommand{\nilv}{\textsf{nil}^{+}}
\newcommand{\nilc}{\textsf{nil}^{-}}
\newcommand{\cons}[2]{#1 :: #2}
\newcommand{\consv}[2]{\textsf{cons}^{+}\left(#1, #2\right)}
\newcommand{\consc}[2]{\textsf{cons}^{-}\left(#1, #2\right)}
\newcommand{\reclist}[5] {
  \textsf{case}\ #1 \textsf{ of }
    \left\{ \, 
      \nil \mapsto #2 
      \mid
      \cons{#3}{#4} \mapsto #5
    \, \right\}
}
\newcommand{\reclistc}[5]{
  \textsf{case}^{-}\left(
      #1 ;
      #2 ;
      (#3, #4).\ #5
  \right)
}
\newcommand{\reclistv}[5]{
  \textsf{case}^{+}\left(
      #1 ;
      #2 ;
      (#3, #4).\ #5
  \right)
}
\newcommand{\pcflist}[1]{\textsf{list}\ #1}
\newcommand{\pcfnil}{\textsf{nil}}
\newcommand{\pcfcons}{\textsf{cons}}
\newcommand{\pcflcase}[5] {
  \textsf{case}\ #1 \textsf{ of }
    \left\{ \, 
      \pcfnil \mapsto #2 
      \mid
      \pcfcons(#3, #4) \mapsto #5
    \, \right\}
}
% \newcommand{\pcflcase}[5]{%
%   \textsf{case}\ #1\ \textsf{of}\ \cbpvnil\Rightarrow #2 \mid 
 %                                  \cbpvcons(#3, #4)\Rightarrow #5}
\WithSuffix\newcommand\pcflcase*[5]{%
  \textsf{case}\ #1\ \textsf{of}\ 
  \begin{aligned}[t]
  &\phantom{{}\mid{}}\pcfnil\mapsto #2 \\
  &{}\mid \pcfcons(#3, #4)\mapsto #5
  \end{aligned}
}

\newcommand{\valbind}[2]{{#1} \leftarrow {#2}}
\newcommand{\pcflet}[2]{%
  \textsf{let}\ {#1}\ \textsf{in}\ {#2}
}
\newcommand{\pcfopm}{\mathbin{\textbf{op}^{+}}}
\newcommand{\pcfopa}{\mathbin{\textbf{op}^{-}}}
\newcommand{\evalpcf}[3]{#1 \downarrow^{#3} #2}
\newcommand{\bounded}[1]{{#1}\mathord{\downarrow}}
\newcommand{\unbounded}[1]{#1\mathord{\uparrow}}

% PCF (recurrence) macros
\newcommand{\cost}{\mathbb{C}}
\newcommand{\costleq}{\leqslant}
\newcommand{\plusc}{\boxplus}
\newcommand{\addcost}{+_{\mathrm{c}}}
\newcommand{\algp}[1]{+_{#1}}
\newcommand{\unitc}{\mathbf{1}}
\newcommand{\zeroc}{\mathbf{0}}
\newcommand{\numc}[1]{\widehat{#1}}
\newcommand{\cbnbisim}{\Mapsto_{\mathrm{cbn}}}
\renewcommand{\max}[2]{\mathop{\mathrm{max}}\left\{#1, #2\right\}}
\newcommand{\maxn}[2]{\mathop{\mathrm{max}_\mathbb{N}}\left\{#1, #2\right\}}
\newcommand{\sem}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\iflor}{\mathbf{if}^\lor}
\newcommand{\semleq}{\preceq}
\newcommand{\rel}[1]{\mathbin{R}_{#1}}
\newcommand{\ectx}[1]{\mathcal{#1}}
\newcommand{\mctx}[1]{\mathcal{#1}}
\newcommand{\mctxtt}[5] % C :: \Gamma |- A \squig \Delta |- B
  { #1 :: \left( #2 \vdash #3 \right) 
            \rightsquigarrow_\textrm{mon.}
          \left( #4 \vdash #5 \right) }
\newcommand{\ectxtt}[5] % C :: \Gamma |- A \squig_elim \Delta |- B
  { #1 :: \left( #2 \vdash #3 \right) 
            \rightsquigarrow _\textrm{elim.}
          \left( #4 \vdash #5 \right) }

% CBPV macros
\newcommand{\eval}[3]{#1 \Downarrow^{#3} #2}
\newcommand{\ct}[1]{\underline{#1}}
\newcommand{\with}{\mathbin{\&}}
\newcommand{\vturn}{\vdash_{\textsf{v}}}
\newcommand{\cturn}{\vdash_{\textsf{c}}}
\newcommand{\thunk}[1]{\textsf{thunk}\ #1}
\newcommand{\force}[1]{\textsf{force}\ #1}
\newcommand{\return}[1]{\textsf{return}\ #1}
\newcommand{\cbpvop}{\mathbin{\textbf{op}}}
\newcommand{\cbpvopm}{\mathbin{\textbf{op}^{+}}}
\newcommand{\cbpvopa}{\mathbin{\textbf{op}^{-}}}
\newcommand{\bind}[3]
  {\textsf{bind} \ #1 \Leftarrow #2\ \textsf{in}\ #3}
\newcommand{\splitprod}[4]{\textsf{split}(#1 ; (#2, #3).\ #4)}
\newcommand{\numl}[1]{\widetilde{#1}}
\newcommand{\calc}[3]
  {\textsf{calc} \ #1 \Leftarrow #2\ \textsf{in}\ #3}
\newcommand{\ifz}[3]
  {\textsf{ifz}(#1 ;\; #2 ;\;  #3)}
\newcommand{\charge}[1]
  {\textsf{charge}.\, #1}
\newcommand{\cbpvlist}[1]{\textsf{list}\ #1}
\newcommand{\cbpvnil}{\textsf{nil}}
\newcommand{\cbpvcons}{\textsf{cons}}
\newcommand{\cbpvlcase}[5]{
  \textsf{case}\left(
      #1 ;
      #2 ;
      (#3, #4).\ #5
  \right)
}
%\newcommand{\cbpvlcase}[5]{%
%  \textsf{case}\ #1\ \textsf{of}\ \cbpvnil\Rightarrow #2 \mid 
%                                  \cbpvcons(#3, #4)\Rightarrow #5}
\WithSuffix\newcommand\cbpvlcase*[5]{%
  \textsf{case}\ #1\ \textsf{of}\ 
  \begin{aligned}[t]
  &\phantom{{}\mid{}}\cbpvnil\Rightarrow #2 \\
  &{}\mid \cbpvcons(#3, #4)\Rightarrow #5
  \end{aligned}
}

% Extraction macros
\newcommand{\logrel}{
  \mathrel{
    \ooalign{\raise.225ex\hbox{$\sqsubset$}\cr\raise-.8ex\hbox{$\sim$}\cr}
  }
}
\newcommand{\valrel}{\logrel^{\mathrm{val}}}
\newcommand{\carrier}[1]{{#1}^\bullet}
\newcommand{\cbnrec}[1]
  {\left\| #1 \right\|} % used for CBN extraction
\newcommand{\cbvrec}[1]
  {\left\| #1 \right\|} % used for CBV extraction (term complexity)
\newcommand{\cbvval}[1]
  {\left\| #1 \right\|} % used for CBV extraction (value complexity)
\newcommand{\cbvpot}[1]
  {\llangle #1 \rrangle}  % used for CBV extraction (potential)
\newcommand{\vrel}[3]{#1 \lesssim^{\mathrm{val}}_{#3} #2}
\newcommand{\crel}[3]{#1 \lesssim^{\mathrm{c}}_{#3} #2}

% Translation macros
\newcommand{\cbvt}[1]{#1^\ast} % CBV-to-CBV
\newcommand{\cbnt}[1]{#1^\dag} % CBN-to-CBPV
\newcommand{\val}[1]{#1^\mathrm{val}} % (CBV-value)-to-(CBPV-value)
\newcommand{\cbpvtv}[4]{#1 \vdash_{\textsf{v}} #2 \searrow #3 : #4} % CBPV-value-to-PCF
\newcommand{\cbpvtc}[4]{#1 \vdash_{\textsf{c}} #2 \searrow #3 : #4} % CBPV-computation-to-PCF
\newcommand{\potential}[1]{\llangle #1 \rrangle}
\newcommand{\complexity}[1]{\left\| #1 \right\|}
\newcommand{\costof}[1]{{#1}_c}
\newcommand{\potentialof}[1]{{#1}_p}

% other macros
\newcommand{\wh}[1]{
  \ifx\hfuzz#1\hfuzz
    \longrightarrow
  \else 
    \longrightarrow_{#1}
  \fi
}

% macros for inductive proofs
\newlist{indproof}{itemize}{5}
\setlist[indproof]{%
%  topsep=30pt,  % space before start / after end of list
  itemsep=5pt,  % space between items
  font={\sc}, % set the label font
  label={}
}
\newcommand{\indcase}[1]{\item{{\sc \color{teal} Case}({\normalfont #1})}.}

\theoremstyle{definition}
\newtheorem{remark}{Remark}


==> pcf-bigstep-lists.tex <==
\vspace{2ex}
    

\begin{tabular}{c c c c}

  \multicolumn{4}{c}{\textbf{Rules for all variants}}

  \\[2ex]

  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \evalpcf{\num{n}}{\num{n}}{0}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \evalpcf{\nil}{\nil}{0}
  \end{prooftree}
  $

  &

  \begin{prooftree}
      \evalpcf{M}{\num{m}}{a}
        \quad
      \evalpcf{N}{\num{n}}{a}
    \justifies
      \evalpcf{M \pcfop N}{\num{m \pcfop n}}{a + b}
  \end{prooftree}

  &

  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \evalpcf{\lambda x.\ M}{\lambda x.\ M}{0}
  \end{prooftree}
  $

  \\[3ex]

\end{tabular}

\begin{tabular}{c c}

  %% IF true
  $
  \begin{prooftree}
      \evalpcf{N}{\num{0}}{a}
        \qquad
      \evalpcf{P}{V}{b}
    \justifies
      \evalpcf{\pif{N}{P}{Q}}{V}{a+b}
  \end{prooftree}
  $

  &

  %% LIST RECURSOR: nil
  $
  \begin{prooftree}
      \evalpcf{L}{\nil}{n}
        \quad
      \evalpcf{M}{V}{m} 
    \justifies
      \evalpcf{\reclist{L}{M}{x}{xs}{N}}
              {V}
              {n + m}
  \end{prooftree}
  $

  \\[3ex]

  %% IF false
  $
  \begin{prooftree}
      \evalpcf{N}{\num{n+1}}{a}
        \qquad
      \evalpcf{Q}{V}{b}
    \justifies
      \evalpcf{\pif{N}{P}{Q}}{V}{a+b}
  \end{prooftree}
  $

  &

  %% LIST RECURSOR: cons
  $
  \begin{prooftree}
      \evalpcf{L}{\cons{H}{T}}{n}
        \quad
      \evalpcf{N[H/x, T/xs]}{V}{m} 
    \justifies
      \evalpcf{\reclist{L}{M}{x}{xs}{N}}
              {V}
              {n + m}
  \end{prooftree}
  $

  \\[4ex]
\end{tabular}

\begin{tabular}{ccc}

  \multicolumn{3}{c}{\textbf{Call-by-name PCF}}

  \\[3ex]

  $
  \begin{prooftree}
      \phantom{no premise}
    \justifies
      \evalpcf{\tuple{M}{N}}{\tuple{M}{N}}{0}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \evalpcf{P}{\tuple{M_1}{M_2}}{a}
        \qquad
      \evalpcf{M_i}{V_i}{b}
    \justifies
      \evalpcf{\pi_i(P)}{V}{a + b + 1}
  \end{prooftree}
  $

  &

  %% CBN FIX
  \multirow{3}{*}{
  $
  \begin{prooftree}
      \evalpcf{M[\fix{x}{M}/x]}{V}{n}
    \justifies
      \evalpcf{\fix{x}{M}}{V}{n + 1}
  \end{prooftree}
  $
  }

  \\[3ex]

  %% CONS
  $
  \begin{prooftree}
      \phantom{\evalpcf{M[\fix{x}{M}/x]}{V}{n}}
    \justifies
      \evalpcf{\cons{H}{T}}{\cons{H}{T}}{0}
  \end{prooftree}
  $

  &

  %% CBN application
  $
  \begin{prooftree}
      \evalpcf{M}{\lambda x.\ P}{m}
        \qquad
      \evalpcf{P[N/x]}{V}{n}
    \justifies
      \evalpcf{M N}{V}{m + n + 1}
  \end{prooftree}
  $

  &

  % empty due to multirow

  \\[4ex]
\end{tabular}

\begin{tabular}{cccc}

  \multicolumn{4}{c}{\textbf{Call-by-value PCF}}

  \\[3ex]

  $
  \begin{prooftree}
      \evalpcf{M}{V}{a}
        \qquad
      \evalpcf{N}{W}{b}
    \justifies
      \evalpcf{\tuple{M}{N}}{\tuple{V}{W}}{a+b}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \evalpcf{P}{\tuple{V_1}{V_2}}{n}
    \justifies
      \evalpcf{\pi_i(P)}{V_i}{n + 1}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \phantom{\evalpcf{H}{V}{n}}
    \justifies
      \evalpcf{\rec{f}{x}{P}}{\rec{f}{x}{P}}{0}
  \end{prooftree}
  $

  &

  $
  \begin{prooftree}
      \evalpcf{H}{V}{n}
        \quad
      \evalpcf{T}{W}{m}
    \justifies
      \evalpcf{\cons{H}{T}}{\cons{V}{W}}{n + m}
  \end{prooftree}
  $

  \\[3ex]

  \multicolumn{4}{c}{
  $
  \begin{prooftree}
      \evalpcf{M}{\lambda x.\ P}{m}
        \qquad
      \evalpcf{N}{W}{n}
        \qquad
      \evalpcf{P[W/x]}{V}{k}
    \justifies
      \evalpcf{M N}{V}{m + n + k + 1}
  \end{prooftree}
  $
  }

  \\[3ex]

  \multicolumn{4}{c}{
  $
  \begin{prooftree}
      \evalpcf{M}{\rec{f}{x}{P}}{m}
        \quad
      \evalpcf{N}{W}{n}
        \quad
      \evalpcf{P[\rec{f}{x}{P}/f, W/x]}{V}{k}
    \justifies
      \evalpcf{M N}{V}{m + n + k + 1}
  \end{prooftree}
  $
  }

\end{tabular}

